Quantum Alphatron: quantum advantage for learning with kernels and noise

At the interface of machine learning and quantum computing, an important question is what distributions can be learned provably with optimal sample complexities and with quantum-accelerated time complexities. In the classical case, Klivans and Goel discussed the \textit{Alphatron}, an algorithm to learn distributions related to kernelized regression, which they also applied to the learning of two-layer neural networks. In this work, we provide quantum versions of the Alphatron in the fault-tolerant setting. In a well-defined learning model, this quantum algorithm is able to provide a polynomial speedup for a large range of parameters of the underlying concept class. We discuss two types of speedups, one for evaluating the kernel matrix and one for evaluating the gradient in the stochastic gradient descent procedure. We also discuss the quantum advantage in the context of learning of two-layer neural networks. Our work contributes to the study of quantum learning with kernels and from samples.

==> QE2abs.tex <==
Large Language Models (or, say, self-supervised learning) from Natural Language Processing are leading the AI revolution. 
Among many applications, they have also been used for those which are also potential applications of quantum computing, like drug design and chemistry. 
As an expected prominent application of quantum computing, Quantum Machine Learning investigates the intersection of ML and quantum computing. 
QML has faced several challenges: 
1. Quantum linear systems based algorithms are hard to realize and require many assumptions on the problem. 
2. It is hard to prove advantage for variational algorithms.  
I will discuss three directions for QML in the age of LLMs. 
(i) Explore the ability of classical methods for quantum data. Here, I will introduce our work on learning of quantum states via operator shadows. 
In addition, I will discuss a result on provable quantum state learning with restricted Boltzmann machines. 
For other directions, I will propose ideas related to,
(ii) Design quantum algorithms in the regime of early fault-tolerant quantum computing, 
and, 
(iii) Build understanding for classical ML from a theoretical point of view.

